Deep Rib Fracture Instance Segmentation and Classification from CT on the RibFrac Challenge

Rib fractures are a common and potentially severe injury that can be challenging and labor-intensive to detect in CT scans. While there have been efforts to address this field, the lack of large-scale annotated datasets and evaluation benchmarks has hindered the development and validation of deep learning algorithms. To address this issue, the RibFrac Challenge was introduced, providing a benchmark dataset of over 5,000 rib fractures from 660 CT scans, with voxel-level instance mask annotations and diagnosis labels for four clinical categories (buckle, nondisplaced, displaced, or segmental). The challenge includes two tracks: a detection (instance segmentation) track evaluated by an FROC-style metric and a classification track evaluated by an F1-style metric. During the MICCAI 2020 challenge period, 243 results were evaluated, and seven teams were invited to participate in the challenge summary. The analysis revealed that several top rib fracture detection solutions achieved performance comparable or even better than human experts. Nevertheless, the current rib fracture classification solutions are hardly clinically applicable, which can be an interesting area in the future. As an active benchmark and research resource, the data and online evaluation of the RibFrac Challenge are available at the challenge website. As an independent contribution, we have also extended our previous internal baseline by incorporating recent advancements in large-scale pretrained networks and point-based rib segmentation techniques. The resulting FracNet+ demonstrates competitive performance in rib fracture detection, which lays a foundation for further research and development in AI-assisted rib fracture detection and diagnosis.

==> fig/froc_post_challenge.tex <==
% !TEX root = ../tmi.tex
% !TEX spellcheck = en-US

\begin{figure}
\centering
\includegraphics[width=\linewidth]{fig/froc_post_challenge_file.pdf}
\caption{\textbf{FROC curves of post-challenge solutions.} They are anonymized as A1, A2 and A3, displayed in solid lines, and compared with top solutions during official challenge period.}
\label{fig:froc_post_challenge}
\end{figure}

==> fig/ribfrac_classes.tex <==
% !TEX root = ../tmi.tex
% !TEX spellcheck = en-US

\begin{figure}
\centering
\includegraphics[width=1.\linewidth]{fig/ribfrac_classes_file.png}
\caption{\textbf{Different classes of rib fractures labelled in the RibFrac dataset.} Other than the four categories presented above, our dataset includes unclassified fractures as well, which are excluded in the evaluation of the classification track.}
\label{fig:ribfrac_classes}
\end{figure}

==> tab/ribfrac_class_num.tex <==
% !TEX root = ../tmi.tex
% !TEX spellcheck = en-US

\begin{table}
    \centering
    \caption{\textbf{Number of different rib fracture categories in the RibFrac training and validation subset.} Four categories of fractures, buckle (BK), non-displaced (ND), displaced (DP) and segmental (SG) are included. Additionally, fractures that are difficult to categorize are labelled as unclassified (UN) and are excluded from the evaluation.}
    \label{tab:ribfrac_class_num}
    \label{tab:ribfrac_dataset_split}
    \begin{tabular}{ccccccc}
        \toprule
        Subset & BK & ND & DP & SG & UN & Total \\
        \midrule
        Training & 618 & 567 & 291 & 179 & 2,332 & 3,987 \\
        Validation & 69 & 63 & 30 & 30 & 243 & 435 \\
        Test & 151 & 188 & 84 & 50 & 409 & 882 \\
        \midrule
        Total & 838 & 818 & 405 & 259 & 2,984 & 5,304 \\
        \bottomrule
    \end{tabular}
\end{table}

